Provable Algorithms for Inference in Topic Models

Recently, there has been considerable progress on designing algorithms with provable guarantees -- typically using linear algebraic methods -- for parameter learning in latent variable models. But designing provable algorithms for inference has proven to be more challenging. Here we take a first step towards provable inference in topic models. We leverage a property of topic models that enables us to construct simple linear estimators for the unknown topic proportions that have small variance, and consequently can work with short documents. Our estimators also correspond to finding an estimate around which the posterior is well-concentrated. We show lower bounds that for shorter documents it can be information theoretically impossible to find the hidden topics. Finally, we give empirical results that demonstrate that our algorithm works on realistic topic models. It yields good solutions on synthetic data and runs in time comparable to a {\em single} iteration of Gibbs sampling.

==> attempt.tex <==
\Tnote{Failure attempts started here}
	We claim that $x_{MLE} \le C\xstar$. For the sake of contradiction, assume this is not true. Then since $\xstar_i \ge \delta/r$, we have that $x_{\mle}\not\in \mathcal B$ where $\mathcal B = B(\xstar,\delta/r, \|\cdot \|_{\infty})$ be the $\delta/r$-infinity norm ball around $\xstar$.    Let $u = \xstar - x_{\mle}$. 
	%Let $\diffmle =z^* -z_{MLE}$. 
	By simple integration along the line of $\diffmle$, we have 
	
	\begin{equation}
	\nabla f(x^*)  = \nabla f(x^*) - \nabla f(x_{\mle}) = \left(\int_{0}^1 \nabla^2 f(t\diffmle)dt \right) \diffmle= -H\diffmle\nonumber
	\end{equation}
	
%		\begin{equation}
%		\nabla g(z^*)  = \nabla g(z^*) - \nabla g(z_{\mle}) = \left(\int_{0}^1 \nabla^2 g(t\diffmle)dt \right) \diffmle= -\widehat{H}\diffmle\nonumber
%		\end{equation}
%		
%		where $\widehat{H} = -\left(\int_{0}^1 \nabla^2 g(t\diffmle)dt \right)$. Let 
		where $H = -\left(\int_{0}^1 \nabla^2 f(t\diffmle)dt \right)$. Let $H_t = -\nabla^2 f(t\diffmle)$, and therefore $H = \int_0^1 H_t dt$.  %Therefore we obtain that $u = -H^{-1}\nabla f(\xstar)  = -H^{-1}Q^{1/2} (Q^{-1/2}\nabla f(\xstar)) = -GQ^{-1/2}\nabla f(\xstar)$, where $G = H^{-1}Q^{1/2}$. 
		
		Let $su+x_{MLE}$ be the point in $\mathcal B$ with maximum $s$. Then for any $1\ge t\ge s$, we have that $tu+x_{\mle}\in \mathcal B$ and therefore $H_t \succeq nQ/4$. It follows that $H =  \int_{0}^1 H_t dt \succeq \int_{s}^1 H_t dt \succeq n(1-s)Q/(4\kappa^2)$. Therefore we obtain that $\|G\|= \|H^{-1}Q^{1/2}\|\le \frac{4\kappa^2}{(1-s)n}$. 
		
		\Tnote{Plan was to show: }
		
		$\|G\|$ is small and therefore $u = G(Q^{-1/2}\nabla f(\xstar))$ has small infinity norm. The problem is that $G$ and $\nabla f(\xstar)$ are not independent. 
		
		\Tnote{Failure attempt ends}

==> beyasian.tex <==
\section{Concentration of the Posterior}

In this section, we show that any algorithm that achieves good estimation error immediately implies a comparable bound on how well the posterior distribution is concentrated. 

Let $y\vert x$ be a model with distribution $p_{y\vert x}$. %Suppose there exists an algorithm 
Suppose $x$ is drawn from prior $p_x$, and $y\vert x$ has distribution $p_{y \vert x}$. Let $p_y$ denotes the marginal density of $y$. For example, when $p_x$ is Dirichlet Prior and $y\vert x$ have distribution $\cat(Ax)$ for some word-topic matrix $A$, this is the LDA model. 
%\Tnote{\cat -- categorical distribution}
%\authnote{RG}{What is $\mbox{Disc}$?}


We will show that the existence of an estimation algorithm with $\epsilon$ estimation bound implies that the concentration of posterior around a ball with radius $\epsilon$. 

\begin{theorem}\label{thm:beyasian}
	Suppose an algorithm $\mathcal{A}$ that takes input $y$ and outputs %(random or deterministic) 
	$\mathcal A(y)$ satisfies that for any $x\in \mathcal{X}$, with probability $1-\delta^2$ over the randomness of $p_{y\vert x}$, it holds that
	\begin{equation}
		\|\mathcal A(y) - x\|\le \epsilon\,.\label{eqn:eqn1}
	\end{equation} 
	Then, for $1-\delta$ fraction of $y$ (with respect to marginal density $p_y$), it holds that the posterior distribution $x\vert y$ is concentrated in a $\epsilon$-ball $\mathcal B(\hat{x},\epsilon)$ for some $\hat{x}$. That is,  
	
	\begin{equation}
		\Pr_{y\vert x}[~\|\hat{x}-x\|\le \epsilon \mid y~]\ge 1-\delta\,.
	\end{equation}

\end{theorem}

\begin{proof}[Proof of Theorem~\ref{thm:beyasian}]
	
	Let $E$ be the event that $\|\mathcal A(y) - x\|\le \epsilon$. By the assumption on algorithm $\mathcal A$ (equation~\ref{eqn:eqn1}) and the law of total expectation, 
	
	\begin{equation}
	\Pr\left[E\right]  = \Pr\left[\Pr\left[E \mid x\right]\right] \ge 1-\delta^2\,.\nonumber
	\end{equation}
	
	Therefore by the law of total expectation, we have 
	
	\begin{equation}
	\Pr\left[E\right]  = \Pr\left[\Pr\left[E \mid y\right]\right] \ge 1-\delta^2\,.\nonumber
	\end{equation}
	
	Then it follows by Markov argument that 
	
	\begin{equation}
 		\Pr\left[\Pr\left[E \mid y\right] \ge 1-\delta \right] \ge 1-\delta\,.\nonumber
	\end{equation}
	
	Note that the inner probability is over the randomness of the posterior distribution $p_{x\mid y}$. Hence, letting $\hat{x} = \mathcal A(y)$, we obtain the desired result.  %and the randomness of $\mathcal A$. 
\end{proof}

Note that Theorem~\ref{thm:beyasian} works for any norm (or more generally any event). For example, based on Theorem~\ref{thm:maininference}, we have
\begin{corollary}
When there are at least $\Omega(\inftybound^2 r^2\log k/\epsilon^2)$ samples, and the prior is uniform on $r$-sparse vectors, then the posterior is concentrated in an $\ell_1$ ball of radius $\epsilon$.
\end{corollary}

==> convexity_old.tex <==
\section{Concavity of the log-likelihood}

Given an observed document $y$, the posterior distribution $x\mid y$ has density function $p[x\vert y] \propto p(y\vert x)p(x)$. Therefore the log-likelihood function can be written as 

\begin{equation}
f(x) =  \sum_{w\in y} \log(\inner{a_{w},x}) - \beta\sum_{i=1}^{k}\log x_i + const
\end{equation}

where $\beta = 1-\alpha\in [0,1]$. %satisfies that $0 \le \beta \le 1$. 

The Hessian of $f$ is: 

\begin{equation}
\nabla^2 f(x)  = -\underbrace{\sum_{w\in y} \frac{a_{w}a_{w}^{\top}}{\inner{a_{w},x}^2}}_{M(x)}+ \beta\diag(x_i^{-2})
\end{equation}

\begin{theorem}\label{thm:lower_bound_M}
	Under assumption~\ref{ass:l_1_condition} and ~\ref{ass:bounded_away}, suppose $N  =  c_0\kappa^2r^2\log k/\delta^2$ for sufficiently large constant $c_0$. Let $M_R(x)$ denote the restriction of $M(x)$ to the indices $R\times R$. Then, with high probability over the randomness of $y$, it holds that for all $x$ such that $ x\le Cx^*$, \begin{equation}
	M_R(x) \succeq N/(2C^2\kappa^2)\cdot \Id_r\,.\label{eqn:psd_lower_bound}
	\end{equation}
\end{theorem}
%Suppose $\supp(x) =  S$ is of size $r$. 

We establish equation~\eqref{eqn:psd_lower_bound} by first showing that with high probability, $M_R(x^*)\ge N/(2\kappa^2)\cdot \Id_r$. Then using the fact that $x\le Cx^*$, we obtain that $M_R(x) \succeq M_R(x^*)/C^2\succeq N/(2C^2\kappa^2)\cdot \Id_r $. Towards obtaining the lower bound for $M_R(x^*)$, we first consider its expectation, which is lowerbounded in the following Lemma. %The following lemma essentially bound the expectation of $\nabla^2 f(x)$. 
\begin{lemma}\label{lem:convexity_expectation}
	%sFor any $x \in \simplex_k$ with $x \le Cx^*$, we have that 
	The expected value of $M(x^*)$ can be lowerbouned by 
%	\begin{equation}
%		\Exp[M(x^*)] = N \sum_{i\in D}  \inner{a_i, x^*} \cdot\frac{a_{i}a_{i}^{\top}}{\inner{a_{i},x}^2}\succeq \frac{N}{C\kappa^2} \cdot \Id_k
%	\end{equation}
	
		\begin{equation}
		\Exp[M(x^*)] = N \sum_{i\in D}  \frac{a_{i}a_{i}^{\top}}{\inner{a_{i},x^*}}\succeq \frac{N}{\kappa^2} \cdot \Id_k\label{eqn:lem:expectation}
		\end{equation}
	where the expectation is over the randomness of the generating process of the document. 
\end{lemma}


\begin{proof}[Proof of Lemma~\ref{lem:convexity_expectation}]
	By definition of the generating process $y\vert x$, we have that 
	\begin{equation}
	\Exp[M(\xstar)] =  N \sum_{i\in [D]} \Pr[w_1 = i]\frac{a_{i}a_{i}^{\top}}{\inner{a_{i},x^*}^2} = N \sum_{i\in [D]}  \frac{a_{i}a_{i}^{\top}}{\inner{a_{i},x^*}} \nonumber
	\end{equation}
	For any unit vector $v\in \R^k$, we consider the quadratic form of $v$ over $\Exp[M(\xstar)]$:
	\begin{align}
	v^{\top} \Exp[M(\xstar)] v %& = N \sum_{i\in [D]} \inner{a_i, x^*}  \cdot \frac{\inner{a_i,v}^2}{\inner{a_{i},x}^2} \nonumber\\
	%& \ge N/C\cdot  \sum_{i\in [D]}\frac{\inner{a_i,v}^2}{\inner{a_{i},x}} \nonumber\\
	& =  N \sum_{i\in [D]}\frac{\inner{a_i,v}^2}{\inner{a_{i},\xstar}}  \nonumber\\
	& =  N \left(\sum_{i\in [D]}\frac{\inner{a_i,v}^2}{\inner{a_{i},\xstar}} \right)\left(\sum_{i \in [D]} \inner{a_i,\xstar}\right) \nonumber\\
	& \ge N\left(\sum_{i\in [D]} \inner{a_i,v}\right)^2 = N \|Av\|_1^2 \nonumber\\
	& \ge N\|v\|_1^2/\kappa^2 \ge N/\kappa^2 \nonumber
	\end{align}
	%where the second inequality uses the fact that $x^*\ge 1/C\cdot x$ and the non-negativity of the entries of $a_i$, $x$ and $x^*$, and 
	where the second line uses the fact that $\sum_i \inner{a_i,\xstar} = 1$, the third line uses Cauchy-Schwartz inequality, and the last line uses that $A$ has $\ell_1$-condition number $\kappa$. (Note that $v$ could take negative entries and therefore $\|Av\|_1$ could be smaller than $\|v\|_1$)
\end{proof}

The following Lemma gives high probability (lower) bound for the spectrum of $M_R(\xstar)$, from which Theorem~\ref{thm:lower_bound_M} follows straightforwardly.  %establish lowerbounds the minimum eigenvalue of $M(x^*)$ with high probability. 
%\begin{proof}[Proof of Lemma~\ref{lem:convexity_expectation}]
%	By definition of the generating process $y\vert x$, we have that 
%	\begin{equation}
%	\Exp[M] =  N \sum_{i\in [D]} \Pr[w_1 = i]\frac{a_{i}a_{i}^{\top}}{\inner{a_{i},x}^2} = N \sum_{i\in [D]} \inner{a_i, x^*}  \cdot \frac{a_{i}a_{i}^{\top}}{\inner{a_{i},x}^2} \nonumber
%	\end{equation}
%	Taking an arbitrary unit vector $v\in \R^k$, we consider the quadratic form of $v$ over $\Exp[M]$:
%	\begin{align}
%		v^{\top} \Exp[M] v& = N \sum_{i\in [D]} \inner{a_i, x^*}  \cdot \frac{\inner{a_i,v}^2}{\inner{a_{i},x}^2} \nonumber\\
%		%& \ge N/C\cdot  \sum_{i\in [D]}\frac{\inner{a_i,v}^2}{\inner{a_{i},x}} \nonumber\\
%				& \ge  N/C\cdot  \left(\sum_{i\in [D]}\frac{\inner{a_i,v}^2}{\inner{a_{i},x}} \right)\left(\sum_i \inner{a_i,x}\right) \nonumber\\
%				& \ge N/C \left(\sum_{i\in [D]} \inner{a_i,v}\right)^2 = N/C \cdot \|Av\|_1^2 \nonumber\\
%				& \ge N/C \cdot \|v\|_1^2/\kappa^2 \ge N/(C\kappa^2). \nonumber
%	\end{align}
%	where the second inequality uses the fact that $x^*\ge 1/C\cdot x$ and the non-negativity of the entries of $a_i$, $x$ and $x^*$, and the fact that $\sum_i \inner{a_i,x} = 1$. 
%	The third line uses Cauchy-Schwartz inequality and the last line uses that $A$ has $\ell_1$-condition number $\kappa$. 
%\end{proof}

\begin{lemma}\label{lem:concentration}
	%Suppose $x \in \simplex_k$ satisfies that $x \le Cx^*$ and $x_i\ge \delta/r$ when $x_i > 0$. 
	Suppose $N  =  c_0\kappa^2r^2/\delta^2\cdot \log k$ for sufficiently large constant $c_0$. Then with probability at least $1-k^{-10}$, we have that 
	\begin{equation}
	M_R(\xstar)\ge N/(2\kappa^2) \cdot \Id_r
	\end{equation}
\end{lemma}
%\Tnote{Some intuition is needed}


Since we have shown that $\Exp[M_R(\xstar)] \succeq  N/\kappa^2\cdot \Id_r$, it would suffice to prove (by matrix concentration inequality) that with high probability, $M_R(\xstar)$ concentrates around its expectation with variance significantly less than $N^2$. However, it turns out that the variance $\Exp[M_R(\xstar)^2]$ could have spectral norm as large as $O(r^4N)$. Then it will require $N \gg r^4$ to guarantee that the spectral norm of the variance can be smaller $N^2$, which turns out to be a suboptimal bound. 

We weaken the requirement to $N \gg r^2$ by observing the following inefficiency in the argument above: Though the variance matrix $\Exp[M_R(\xstar)^2]$ could have a large eigenvalue with some eigenvector $v$, when this happens the expectation $\Exp[M_R(\xstar)]$ also have eigenvalue much larger than $N/\kappa^2$ around some direction correlated with $v$ (in the meantime it might also have a small eigenvalue $N/\kappa^2$ in some other direction so that the lower bound $\Exp[M_R(\xstar)] \succeq  N/\kappa^2\cdot \Id_r$ cannot be improved). This suggests us to first whiten the expectation matrix to identity matrix, so that we can avoid the inefficiency caused by using spectral norm to measure the size of a very skew matrix. 
\begin{proof}[Proof of Lemma~\ref{lem:concentration}]
	

Let $\hata_w\in \R^r$ be the restriction of $a_w$ to the support $R$. 
For $w\in y$, let $Z_w  = \frac{\hata_{w}\hata_{w}^{\top}}{\inner{\hata_{w},\xstar}^2}$. Let $Q = \sum_{i\in [D]}  \frac{\hata_{i}\hata_{i}^{\top}}{\inner{\hata_{i},x^*}}$. By Lemma~\ref{lem:convexity_expectation}, we have that $M_R(\xstar) = \sum_{w\in y} Z_w$ and $\Exp[M_R(\xstar)] = NQ$. Moreover, since $Q = \Exp[M_R(\xstar)]$ is the restriction of $\Exp[M(\xstar)]$ to the indices $R\times R$, by equation~\eqref{eqn:lem:expectation}, we have that $Q \succeq 1/\kappa^2\cdot \Id_r$. 



%For simplicity, for any $j\in [N]$, let $Z_j = \frac{a_{w_j}a_{w_j}^{\top}}{\inner{a_{w_j},x}^2}$. Let $Q = \Exp[Z_1]= \frac{a_{i}a_{i}^{\top}}{\inner{a_{i},x}^2}\succeq \frac{N}{C\kappa^2}$. 

Let $Z'_w = Q^{-1/2}Z_wQ^{-1/2}$. Consider the random variable $M'\in \R^{r\times r}$, which is a sum of independent random matrices, 
\begin{equation}
M' = \sum_{w\in y}Z_w' \nonumber
\end{equation}

Toward bounding the fluctuation of $M'$, we apply Bernstein inequality~\cite{} on $M'$. 
% %First, since $Z_j \preceq \frac{\|a_{w_j}\|_2^2}{\inner{a_{w_j},x}^2}$ 
By Lemma~\ref{lem: tech_lem_1}, we know that $\left\|Z_w\right\| \le r^2/\delta^2$. Then 
\begin{equation}
Z_w' = Q^{-1/2}Z_wQ^{-1/2} \preceq Q^{-1/2} \cdot r^2/\delta^2\Id_r \cdot Q^{-1/2} = r^2/\delta^2 \cdot Q^{-1}\nonumber
\end{equation}

Therefore it follows that $\left\|Z_w'\right\| \le r^2/\delta^2 \|Q^{-1}\| \le r^2 \kappa^2/\delta^2$. 

Next we  bound the variance of $M'$: %First we have that 
\begin{align}
\Exp[(Z_w')^2] & =  \sum_{i\in [D]} \inner{a_i, x^*}  \cdot \left(Q^{-1/2}\frac{\hata_{i}\hata_{i}^{\top}}{\inner{\hata_{i},\xstar}^2}Q^{-1/2} \right)^2\nonumber \\
& =  \sum_{i\in [D]} \frac{\hata_i^{\top}Q^{-1}\hata_i}{\inner{\hata_i,\xstar}^2}\cdot  Q^{-1/2}\frac{\hata_{i}\hata_{i}^{\top}}{\inner{\hata_{i},\xstar}}Q^{-1/2} \nonumber \\
& \preceq \sum_{i\in [D]} \frac{\|\hata_i\|_2^2 \|Q^{-1}\|}{\inner{\hata_i,\xstar}^2}\cdot  Q^{-1/2}\frac{\hata_{i}\hata_{i}^{\top}}{\inner{\hata_{i},\xstar}}Q^{-1/2} \nonumber \\
%& \preceq  \sum_{i\in [D]} \inner{a_i, x^*} \cdot \frac{C\kappa^2 r^2/\delta^2}{\inner{a_i,x}^2}\cdot Q^{-1/2} \frac{a_{i}a_{i}^{\top}}{\inner{a_{i},x}^2}Q^{-1/2} \nonumber \\
& \preceq 1/\kappa^2 \cdot r^2/\delta^2 \cdot \sum_{i\in [D]}Q^{-1/2}\frac{\hata_{i}\hata_{i}^{\top}}{\inner{\hata_{i},\xstar}}Q^{-1/2}  \nonumber\\
& = \kappa^2 \cdot r^2/\delta^2 \cdot  Q^{-1/2}QQ^{-1/2}  = \kappa^2r^2/\delta^2 \cdot \Id_r\nonumber
%& = \kappa^2 r^2/\delta^2Q^{-1/2}QQ^{-1/2} = C\kappa^2 r^2/\delta^2\Id_r
\cdot 
%\frac{\|a_i\|_2^2 a_ia_i^{\top}}{\inner{a_{i},x}^4}
\end{align} 

where the second line uses the fact that $\supp(\xstar)  =R$ and therefore $\inner{a_i,\xstar} = \inner{\hata_i,\xstar}$, and the  third line uses the definition of spectral norm, and the fourth line uses Lemma~\ref{lem: tech_lem_1} and $Q\ge 1/\kappa^2 \cdot \Id_r$, and finally the fifth line uses the definition of $Q$. 

%Therefore we have that $\left\|\Exp[\sum_j (Z_j')^2] \right\|\le N$. 

Now we are ready to apply Bernstein inequality on $M'$. We conclude that with high probability,  %we have that with high probability, it holds that 

\begin{equation}
\left\|M' - \Exp[M']\right\| \le O(\sqrt{\kappa^2 r^2/\delta^2\cdot N\log k} + r^2\kappa^2/\delta^2\cdot \log k)\nonumber
\end{equation}

Recall the definition of $M' = Q^{-1/2} \Exp[M_R(\xstar)]Q^{-1/2}$, we obtain that for $N\ge c_0r^2\kappa^2/\delta^2\cdot \log k$ with sufficiently large constant $c_0$, 

\begin{equation}
 - N/2\cdot \Id_r \preceq Q^{-1/2} \left(M_R(\xstar) - \Exp[M_R(\xstar)]\right) Q^{-1/2} \preceq N/2\cdot \Id_r\nonumber
\end{equation}

It follows that $M_R(\xstar) -\Exp[M_R(\xstar)] \succeq -N/2 \cdot Q$. Recall that $\Exp_R[M(\xstar)] = NQ$. Therefore, equation above implies that

%It follows $\Exp[M] = Q$ that 

\begin{equation}
M_R(\xstar) \succeq N/2\cdot Q \nonumber%\succeq %(N - O(\sqrt{C\kappa^2 r^2/\delta^2N\log k} + r^2C\kappa^2/\delta^2\log k)) Q\nonumber
\end{equation}
which in turn implies that \begin{equation}
M_R(\xstar) \succeq N/2\cdot Q \succeq N/(2\kappa^2) \cdot \Id_r\nonumber
\end{equation}
%for some $N = O(C\kappa^2r^2\log k/\delta^2)$. 
\end{proof}
\begin{lemma}\label{lem: tech_lem_1}
	Suppose  $x\in \simplex_k$ and  $\forall i, x_i\ge \delta/r$ if $x_i > 0$. Then for any vector $a\in \R_{\ge 0}^k$, $\|a_R\|_2 \le \delta/R\cdot \inner{a,x}$ and $\left\|\frac{a_Ra_R^{\top}}{\inner{a,x}^2}\right\| \le r^2/\delta^2$. 
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem: tech_lem_1}]
	Let $R$ be the support of $x$. Then we have that $\inner{a,x} \ge \delta/r \cdot \|a_R\|_1 \ge \delta/r \|a_R\|_2$, and therefore $\left\|\frac{a_Ra_R^{\top}}{\inner{a,x}^2}\right\| \le \frac{\|a_R\|_2^2}{\inner{a,x}^2}\le r^2/\delta^2$. 
\end{proof}

==> intro1.tex <==
\section{Introduction}

%\subsection{Background}

 Generative models of data are ubiquitous in machine learning. ncluding topic models, mixture models, hidden markov models, stochastic block models and graphical models. Of course, no model can ever hope to be perfectly accurate and is at best a simplification of some much more complicated process that generated the data. Regardless, given a generative model there are two basic questions that we can ask: (1) In parameter learning the goal is to find the parameters that describe which particular model from the family was used to generate the data. (2) And in inference, we are given the parameters of the model and our goal is to compute the posterior distribution -- e.g. given a sample, what is the posterior distribution on clusters on which it came from? 

Recently, there has been considerable interest in designing algorithms with provable guarantees for parameter learning. In many cases, just a few years ago we had only heuristics where it was difficult to analyze when and why they worked. But recently, several groups of researchers have given algorithms that provable work --- they run in polynomial time and require a polynomial number of samples --- for learning the parameters of topic models, mixture models, stochastic block models, independent component analysis and deep learning. In many of these settings, computing the maximum likelihood estimate is NP-hard. But these results work around this obstacle, by designing alternate estimators based on tensor decompositions, the method of moments or other ad hoc approaches, that converge to the true parameters at an inverse polynomial rate and yet can be computed provable and efficiently.


Often, what we want to do with the parameters is perform inference. Let's consider the example of topic modeling since it will be our main focus in this paper. Here we are given a collection of documents each of which is represented as a {\em bag of words}. The central assumption is that there is a fixed set of {\em topics} that are shared and recur in different proportions in each document. Each topic is itself a distribution on words. Then each document is generated by first picking its topic proportions from some distribution, and then sampling each word from the document-specific distribution on words. The goal in parameter learning is to learn the topics from the collection of documents. These topics are already useful for summarization. In fact one of their main uses is for inference. Given the topics, can we compute infer the topic proportions in a given document? If we could compute this, we could do more than just summarize. We could classify and categorize each document in the collection. 

The trouble is that in many settings inference appears to be much harder than parameter learning. Even though there are many known algorithms with provable guarantees for learning the parameters of a topic model, to the best of our knowledge there are no known algorithms with provable guarantees for inference in these settings. What is even more confounding is that heuristics like Gibbs sampling (which are notoriously difficult to analyze and give provable guarantees for) attempt to do both parameter learning and inference simultaneously. 

It is not hard to come up with contrived examples where parameter learning is computationally easy, but inference is hard. In fact, another way to understand the difference between these two types of problems is that in parameter learning one need not make information theoretically optimal use of the samples, whereas in inference ignoring even a handful of words in a long document could drastically affect the posterior distribution on its topics.

\subsection{Our Results}

Here we give the first algorithms with provable guarantees for inference in topic models. Our first goal is to compute an estimate for the topic proportions that is accurate in $\ell_1$-distance. We work with the usual generative model where there is an underlying word-by-topic matrix $A$ whose columns represent topics and are themselves distributions on words. Instead of generating a document as a mixture of topics by sampling a vector from the Dirichlet distribution, we will explicitly assume that each document is an $r$-sparse mixture of topics. %whe. %We will posit a distribution on $r$-sparse vectors, and then 
With the topic proportions $\xstar$ fixed, $n$ words are sampled independently from the multinomial distribution defined by $A\xstar$ to form the document $y$. We will use $y$ interchangeably to denote the set of words or the count vector of the words in the document. 

%\Tnote{In most parts of this I guess we don't  need a particular prior}
\Tnote{Edited above. Maybe we should say we take frequentist point of view explicitly?}

\Tnote{Maybe it'd better to desribe the model in a bit more detail?}

\Tnote{We might need to be a bit careful about the use of $\xstar$, $x$ and $\hat{x}$ in this section. }

We work with various notions of the condition number that are appropriate for matrices whose columns have unit $\ell_1$-norm as is the case in topic modeling. We introduce these later, but we find that empirically in most applications these condition numbers are bounded by a small constant --- say $1.5$ or $2$. One such condition number was introduced by Kleinberg and Sandler~\cite{KleinbergS08}, who gave applications of it to collaborative filtering. The notion of condition number we introduce is actually a relaxation --- i.e. it is always smaller --- but nevertheless we can show that it is equivalent to the existence of a good linear estimator for the topic proportions that itself has small variance. 

\begin{theorem}
	\label{thm:maininference-intro}
	Suppose $A$ has good condition number, then there exists a matrix $B$ and threshold $\tau$ such that the simple estimator $x = \threshold_{\tau}(By/n)$ satisfies that: given documents of $n = O(r^2\log k)$ words, with high probability $x$ has distance $c$ in $\ell_1$ norm and distance $c/r$ in $\ell_{\infty}$ norm to $\xstar$.  
	%If the original vector $x^*$ is an $r$-sparse vector, for any $\epsilon > 4\delta r$, given $n = \Omega(\inftybound^2 r^2 \log k/\epsilon^2)$ samples, with high probability Algorithm~\ref{alg:inference} returns a vector that has $\ell_1$-distance at most $\epsilon$ with $x^*$.
\end{theorem}

Thus we can recover the set of topics present in the document when the document has length about $r^2$, provided that the condition number of $A$ is appropriately bounded. In comparison, if we were to consider {\em very long} documents then the empirical distribution on words would be a good approximation to $A\xstar$ and we could left multiply by the pseudo-inverse of $A$ to obtain $\xstar$ almost exactly, independently of whether or not it is sparse. The trouble is that this estimator has a much larger variance than does ours, and that is what allows us to work with much shorter documents. Of course, the same two-level generative model is used not only in topic modeling but also in collaborative filtering, and there our results allow us to make accurate predictions about users that have rated purchased very few items, compared to what was known before. 

We also adopt a Bayesian perspective. Here, instead of being interested in obtaining an estimate for $\xstar$ that is close in $\ell_1$ distance we might instead be interested in sampling from the posterior distribution on $x$ given the words we have observed. This type of goal is most natural when the posterior distribution is somewhat concentrated, and we show a general result that an algorithm for learning $x$ with respect to some metric immediately implies that the posterior on $x$ concentrates at roughly the same scale. 

\begin{theorem}\label{thm:beyasian-intro}
	Suppose there exists an algorithm $\mathcal A$ that takes observation $y$ (from model $p(y\vert x)$) and is guaranteed to output an estimate $\hatx$ of the hidden variable such that with high probability $\hatx$ has $\epsilon$ estimation error in some norm $\|\cdot \|$. Then for any prior $p(x)$ and joint distribution $p(x,y) = p(y\vert x)p(x)$, with high probability over the marginal distribution of $y$, it holds that the posterior distribution $p(x\vert y)$ is concentrated (with high probability mass) around a ball with radius $\epsilon$ with respect to norm $\|\cdot \|$. 

	
	
%	Given a generative model with joint distribution $p(x,y)$. 
%	Suppose an algorithm $\mathcal{A}$ that takes input $y$ and outputs %(random or deterministic) 
%	$\mathcal A(y)$ satisfies that for any $x\in \mathcal{X}$, with probability $1-\delta^2$ over the randomness of $p_{y\vert x}$, it holds that
%	\begin{equation}
%	\|\mathcal A(y) - x\|\le \epsilon\,.\label{eqn:eqn1}
%	\end{equation} 
%	Then, for $1-\delta$ fraction of $y$ (with respect to marginal density $p_y$), it holds that the posterior distribution $x\vert y$ is concentrated in a $\epsilon$-ball $\mathcal B(\hat{x},\epsilon)$ for some $\hat{x}$. That is,  
%	
%	\begin{equation}
%	\Pr_{y\vert x}[~\|\hat{x}-x\|\le \epsilon \mid y~]\ge 1-\delta\,.
%	\end{equation}
%	
\end{theorem}

We complement these results by showing that even when the condition number is bounded, information theoretically it is impossible to recover the support of the distribution on topics with documents that are shorter than $r^2$ words. 

\begin{theorem}\label{thm:lower_bound_intro}
	There exists a (distribution of) word topic matrix $A$ with condition number close to 1 such that any algorithm $\mathcal A$ that takes document of $o(r^2)$ words as input cannot recover, with probability at least $3/4$,  the support of the topic vector $\xstar$ that is used to generate $y$ . This is still true when $\xstar$ is promised to have only non-zero entries that are larger than $1/r$. 
\end{theorem}

We also show that once we have learned the support of $x$ it is possible to perform gradient ascent on the likelihood function, and obtain an even better rate of convergence. 

\Tnote{Just reminder: $\ell_1\rightarrow\ell_1$ condition number is not defined yet. }

\begin{theorem}\label{thm:rate_intro}
	%\Tnote{Missing the condition on $n$}
	%Under assumption~\ref{ass:bounded_away} and~\ref{ass:restricted_ell_1}, suppose $n\ge c\kappa^2r^2\log k/\ltau^2$ for a sufficiently large constant $c$.
	Let $x_{\mle}$ be the maximizer of the log-likelihood function %$f(x)$ 
	restricted to support $R$ of $\xstar$. Suppose $A$ has good restricted $\ell_1\rightarrow \ell_1$ condition number and $\xstar$ have non-zero entries bounded away from zero. Then, with high probability $x_{\mle}$ has prediction error and estimation error, 
	\begin{equation}
	\|Ax_{\mle} - A\xstar\|_1 \le \widetilde{O}\left(\sqrt{\frac{r}{n}}\right)\,,\nonumber
	\end{equation}
	and 
	\begin{equation}
	\|x_{\mle} - \xstar\|_1\le \widetilde{O}\left(\kappa\sqrt{\frac{r}{n}}\right) \mper \nonumber
	\end{equation}
\end{theorem} 

\Tnote{Not sure how to say the rate is optimal -- we believe it is. }

It turns out that this hybrid type of algorithm, that uses a suitably chosen linear estimator (where we solve a convex program to find the estimator with the smallest possible variance) and then performs gradient ascent achieves better performance than either approach alone. We run our algorithms on a collection of synthetic datasets and compare to Gibbs sampling. We show that our algorithms obtain comparable recovery guarantees, while being much faster (since they are based on elementary linear algebraic steps as opposed to running a markov chain and waiting for it to mix). 

\Tnote{Maybe mention that our problem is the $\ell_1$ counter part of the sparse linear regression problem which have been studied extensively. There are two difficulties here -- a) the noise model is not nice (compared to Gaussian) since the generative model involves sampling from category distribution.  b) In especially the analysis of MLE, since the MLE is asymptotically Gaussian and therefore the natural norm to study it needs to be $\ell_2$. To get tight bound, it's necessary to use the fisher information matrix to change the $\ell_1$ norm space to $\ell_2$ carefully. }


==> likelihood_hold.tex <==
\section{Likelihood of the linear inverse}

In this section we try to show the result we get from the linear inverse has good log-likelihood in expectation.

We will still use Assumption~\ref{ass:bounded_away}. We will represent the document $y$ as a $D$-dimensional vector (recall $D$ is the size of the vocabulary), and let $x$ be the recovered topic proportions. The (negative) log-likelihood is equal to
$$
L(y) = - \sum_{i=1}^D y_i \log (Ax)_i.
$$

Here $x$ is a function of $y$, however, the following claim shows when we have enough samples the variables in the log are concentrated:

\begin{claim}
If we have $\tilde{O}(r^2/\delta^2\epsilon^2)$ samples, with high probability the recovered $x$ has the same support as $x^*$, and $|x_i - x^*_i|\le \epsilon\delta r \le \epsilon x^*_i$.
\end{claim}

This means $|\log (Ax)_i - \log (Ax^*)_i| \le \epsilon$ with high probability. Therefore

$$
\E[L(y)] = - \E[\sum_{i=1}^D y_i (\log(Ax^*)_i \pm \epsilon)]
= - N \sum_{i=1}^D (Ax^*)_i(\log(Ax^*)_i \pm \epsilon N.
$$

The first term is the optimal log-likelihood, and we are off by only $\epsilon N$ (notice that $\epsilon = \sqrt{r^2/\delta^2 N}$ so the true error is $O(r\sqrt{N}/\delta)$), which is a lower order term.


Also, the ``expectation'' here is a bit strange: in inference (or MLE) we are allowed to choose an optimal $x$ for every document $y$. On the other hand, when we say our log-likelihood is within an additive factor of $\epsilon N$, we are comparing against the best possible solution that gives the same decoding $x^*$ to every $y$ in this distribution. 

%In order to really prove the decoded $x$ is approximately optimal, we need the following Conjecture:
%\begin{claim}
%With high probability over $y$, $$\sup_x \sum_{i=1}^D y_i\log x \approx N \sum_{i=1}^D (Ax^*)_i \log (Ax^*)_i.$$
%\end{claim}
%
%This seems correct and may follow from some VC-dimension like proof (the fact that there are only $r$ dimensions in $x$).

Next we will prove that the true log-likelihood is concentrated around the expectation. In order to avoid taking the $\log$ of 0 we use the standard {\em smoothing} technique and use $\log \max\{1/k^2, (Ax)_i\}$. This can be interpreted as assigning $1/k$ mass uniformly to all topics.

\begin{lemma}
With high probability, for any $r$-sparse vector $x$, we have

$$
|\sum_{i=1}^D y_i \log \max\{1/k^2, (Ax)_i\} - N \sum_{i=1}^D (Ax^*)_i \log \max\{1/k^2, (Ax)_i\}|
\le \tilde{O}(\sqrt{rN})
$$
(where $\tilde{O}$ hides $\log k$ factors)
\end{lemma}

\begin{proof} (sketch)
Basically just need to take union bound over an $\epsilon$ net for $r$-sparse vectors (the net has size $(k/\epsilon)^{O(r)}$). The smoothing provides a infinity norm on the coefficients which allows us to use Bernstein's inequality for each $x$ in the net.
\end{proof}

Notice that the lemma above does not require the lowerbound on the $x^*$ entries! This gives us a way to utilize the $\ell_1$ condition number: let
$$
T(x) = N \sum_{i=1}^D (Ax^*)_i \log \max\{1/k^2, (Ax)_i\},
$$
we know $T(x)$ is close to the log likelihood for {\em every} $x$. On the other hand, we know $x^*$ is the optimal for $T(x)$ and

$$
T(x) - T(x^*) = N\cdot KL(Ax, Ax^*) \ge 2N |Ax-Ax^*|_1^2 \ge \frac{2}{\kappa^2} |x-x^*|_1^2.
$$

This in particular means if $|x-x^*|_1$ is large (larger than $\tilde{\Omega}((N/r)^{-1/2})$), the probability of $x$ will be super small and can be ignored. Therefore we only need to restrict our attention to vectors that have $\ell_1$ norm at most $\tilde{O}((N/r)^{-1/2})$. 

The remaining problem: there are still many possible vectors that is within this $\ell_1$-distance to the decoded $x$, and they can have many possible supports. How do we sample from them?

==> likelihood_old.tex <==
\section{Likelihood of the linear inverse}

In this section we try to show the result we get from the linear inverse has good log-likelihood in expectation.

We will still use Assumption~\ref{ass:bounded_away}. We will represent the document $y$ as a $D$-dimensional vector (recall $D$ is the size of the vocabulary), and let $x$ be the recovered topic proportions. The (negative) log-likelihood is equal to
$$
L(y) = - \sum_{i=1}^D y_i \log (Ax)_i.
$$

Here $x$ is a function of $y$, however, the following claim shows when we have enough samples the variables in the log are concentrated:

\begin{claim}
If we have $\tilde{O}(r^2/\delta^2\epsilon^2)$ samples, with high probability the recovered $x$ has the same support as $x^*$, and $|x_i - x^*_i|\le \epsilon\delta r \le \epsilon x^*_i$.
\end{claim}

This means $|\log (Ax)_i - \log (Ax^*)_i| \le \epsilon$ with high probability. Therefore

$$
\E[L(y)] = - \E[\sum_{i=1}^D y_i (\log(Ax^*)_i \pm \epsilon)]
= - N \sum_{i=1}^D (Ax^*)_i(\log(Ax^*)_i \pm \epsilon N.
$$

The first term is the optimal log-likelihood, and we are off by only $\epsilon N$ (notice that $\epsilon = \sqrt{r^2/\delta^2 N}$ so the true error is $O(r\sqrt{N}/\delta)$), which is a lower order term.


Also, the ``expectation'' here is a bit strange: in inference (or MLE) we are allowed to choose an optimal $x$ for every document $y$. On the other hand, when we say our log-likelihood is within an additive factor of $\epsilon N$, we are comparing against the best possible solution that gives the same decoding $x^*$ to every $y$ in this distribution. 

%In order to really prove the decoded $x$ is approximately optimal, we need the following Conjecture:
%\begin{claim}
%With high probability over $y$, $$\sup_x \sum_{i=1}^D y_i\log x \approx N \sum_{i=1}^D (Ax^*)_i \log (Ax^*)_i.$$
%\end{claim}
%
%This seems correct and may follow from some VC-dimension like proof (the fact that there are only $r$ dimensions in $x$).

Next we will prove that the true log-likelihood is concentrated around the expectation. In order to avoid taking the $\log$ of 0 we use the standard {\em smoothing} technique and use $\log \max\{1/k^2, (Ax)_i\}$. This can be interpreted as assigning $1/k$ mass uniformly to all topics.

\begin{lemma}
With high probability, for any $r$-sparse vector $x$, we have

$$
|\sum_{i=1}^D y_i \log \max\{1/k^2, (Ax)_i\} - N \sum_{i=1}^D (Ax^*)_i \log \max\{1/k^2, (Ax)_i\}|
\le \tilde{O}(\sqrt{rN})
$$
(where $\tilde{O}$ hides $\log k$ factors)
\end{lemma}

\begin{proof} (sketch)
Basically just need to take union bound over an $\epsilon$ net for $r$-sparse vectors (the net has size $(k/\epsilon)^{O(r)}$). The smoothing provides a infinity norm on the coefficients which allows us to use Bernstein's inequality for each $x$ in the net.
\end{proof}

Notice that the lemma above does not require the lowerbound on the $x^*$ entries! This gives us a way to utilize the $\ell_1$ condition number: let
$$
T(x) = N \sum_{i=1}^D (Ax^*)_i \log \max\{1/k^2, (Ax)_i\},
$$
we know $T(x)$ is close to the log likelihood for {\em every} $x$. On the other hand, we know $x^*$ is the optimal for $T(x)$ and

$$
T(x) - T(x^*) = N\cdot KL(Ax, Ax^*) \ge 2N |Ax-Ax^*|_1^2 \ge \frac{2}{\kappa^2} |x-x^*|_1^2.
$$

This in particular means if $|x-x^*|_1$ is large (larger than $\tilde{\Omega}((N/r)^{-1/2})$), the probability of $x$ will be super small and can be ignored. Therefore we only need to restrict our attention to vectors that have $\ell_1$ norm at most $\tilde{O}((N/r)^{-1/2})$. 

The remaining problem: there are still many possible vectors that is within this $\ell_1$-distance to the decoded $x$, and they can have many possible supports. How do we sample from them?

==> old_proofs.tex <==
\section{Old proofs}


\begin{lemma}
	Suppose $x^* \le C'x$ and $x_i \ge \delta/r$ for non-zero $x_i$. Let \begin{equation}
	\sigma^2 = \left\|\Exp\left[\sum_{j\in [N]} \frac{\|a_{w_j}\|_2^2 a_{w_j}a_{w_j}^{\top}}{\inner{a_{w_j},x}^4}\right] \right\|= N\left\|\sum_{i\in [D]} \inner{a_i, x^*}  \cdot \frac{\|a_i\|_2^2 a_ia_i^{\top}}{\inner{a_{i},x}^4}\right\|
	\end{equation}
	be the variance term for applying bernstein inequality for $M$. 
	Then 
	$$\sigma^2 \le O(C'N r^4/\delta^4)\cdot \max_i \frac{\|a_i\|_2^4}{\|a_i\|_1^4} \le O(C'Nr^4/\delta^4)$$
\end{lemma}

\begin{proof}
	\begin{align}
		\sigma^2 &\le  
		\sum_{i\in [D]} \inner{a_i, x^*}  \cdot \frac{\|a_i\|_2^4}{\inner{a_{i},x}^4} \nonumber\\
		& \le C'\sum_{i\in [D]} \inner{a_i,x} \cdot \frac{\|a_i\|_2^4}{\inner{a_{i},x}^4}\nonumber\\
				& \le C'\sum_{i\in [D]} \inner{a_i,x} \cdot \frac{\|a_i\|_2^4}{\delta^4/r^4 \cdot \|a_i\|_1^4 } \nonumber\\
				& \le O(C'N r^4/\delta^4) \sum_{i\in [D]} \inner{a_i,x} = O(C'N r^4/\delta^4) \nonumber
	\end{align}
\end{proof}


==> toolbox.tex <==
\section{Toolbox}

\begin{theorem}\label{thm:bernstein}
	[Matrix Bernstein, \cite[Thm.~6]{Gross11},~\cite[Thm.~3.2]{Recht11}, ~\cite[Thm.~1.5]{Tropp2011}] 
	Consider a finite sequence $\{ X_k \}$ of independent, random  matrices with dimension $d_1\times d_2$.  Assume that each random matrix satisfies
	$$
	\|X_k- \Exp[X_k]\| \leq R
	\quad\text{almost surely}.
	$$
	Then, for all $t \geq 0$,
	$$
	\Pr\left[\left\| \sum\nolimits_k X_k - \Exp\left[\sum\nolimits_k X_k\right]\right\|  \geq t\right] 
	\leq (d_1+d_2) \cdot \exp\left( \frac{-t^2/2}{\sigma^2 + Rt/3} \right)
	$$
	where 
$$
	\sigma^2 := \max\{\left\| \sum\nolimits_k \Exp\left[X_kX_k^{\top}\right] \right\|, \left\| \sum\nolimits_k \Exp\left[X_k^{\top}X_k\right] \right\| \}$$
\end{theorem}
